A Mathematical Theory of Attention

Attention is a powerful component of modern neural networks across a wide variety of domains. However, despite its ubiquity in machine learning, there is a gap in our understanding of attention from a theoretical point of view. We propose a framework to fill this gap by building a mathematically equivalent model of attention using measure theory. With this model, we are able to interpret self-attention as a system of self-interacting particles, we shed light on self-attention from a maximum entropy perspective, and we show that attention is actually Lipschitz-continuous (with an appropriate metric) under suitable assumptions. We then apply these insights to the problem of mis-specified input data; infinitely-deep, weight-sharing self-attention networks; and more general Lipschitz estimates for a specific type of attention studied in concurrent work.

==> main_structured.tex <==
\section{Structured Data, and Random Fields, and Measures}
\remi{Wondering whether this section should be merged with Notations and preliminaries}
\aristide{In fact I would even move the current Sec 1.1 to the Appendix (and/or release the defs on the fly in text) and replace it by this Section 3}\remi{I'm fine with the Markov kernel part of the notations. Agreed about the more mainstream definitions like TV and KL}\james{Make a precise definition of structured data}
In this section, we consider the problem of unifying the treatment of ``structured data'' by an attention based model. We consider structured data to be collections of distinct elements together with some structure describing their relationships. Text, graphs, and images all fit neatly within this very broad description, and our first task is to show how these three modalities are instances of random fields. Then we will show how to associate to these structured data a measure, and how ``features'' of these data are represented.

\subsection{Structured Data}
\james{Structured data is any data which can be modelled by a random field.}
\begin{definition}[Random Field]
	Let $(\Omega,\calF,\P)$ be a probability space. Let $\calT$ be a topological space. Let $(S,\calS)$ be a measurable state space. A random field $\mbf{x}$ is a collection of random variables on $\Omega$ indexed by $\calT$, i.e. $\mbf{x}=\{x_t\}_{t\in \calT}$ where $x_t:\Omega\to S$.
\end{definition}
In this paper, we will assume that $\calT$ and $S$ are discrete, finite sets. For statistical modelling, we are interested in approximating the law of $\mbf{x}$, denoted $P:=\mbf{x}_*\P$, by another measure $Q$. Moreover, we will assume the existence of a neighbourhood mapping $\calN:\calT\to 2^\calT$ such that
\[
	P(x_t|\mbf{x}_{-t}) = P(x_t | \calN(t)).
\]where we have used $-t:=\calT\setminus\{t\}$. In general, this imposes no restrictions on $P$ since $\calN(t)$ can be arbitrary and it is a result due to \cite{besag1974spatial} that knowledge of the complete conditionals is sufficient to uniquely determine the joint law. On the other hand, statistical modelling text, graphs, and images are instances of modelling such a law, therefore we will consider random field modelling in the remainder of this paper.

\subsection{Measures \& Features}
\label{sub:features}
The nature of self-attention, as we will see below, is best\james{don't use superlatives w/o justification} modelled as a measure-transport phenomenon. Therefore, in preparation for this, we establish some key concepts.

Firstly, we define the empirical measure mapping. Let $E\in \calB(\R^d)$ be a Borel-measurable subset. There is a natural bijection between $E$ and $\calP_\delta(E):=\{\delta_x\st x\in E\}$ induced by the mapping
\[
	x\mapsto \delta_x.
\]This way, we can associate any random field with state space $S\subset E$ to a measure in $\calP(E)$:
\[
	\mbf{x}\mapsto m(\mbf{x}):=\frac{1}{|\calT|}\sum_{t\in \calT} \delta_{x_t}.
\]{\todo this mapping is not exchangeable} This mapping appears to be the ``right'' setting for studying the action of self-attention.\remi{Justify, or say something like: As we will see later, this setting allows us to model self-attention as an object acting on measures amenable to self-composition blabla.} We also define the inverse mapping on the set of uniform empirical measure: $m^{-1}(\frac{1}{|\calT|}\sum_{t\in \calT} \delta_{x_t}) = (x_t)_{t \in \calT}$.


Secondly, we establish the concept of a feature encoded in a measure\remi{Is this a classic way of doing things? If so, reference?}. Let $F:E\to E'\subset \R^{d'}$ be a measurable map, representing a feature extractor \james{terrible terminology}. We say that a measure $\mu\in \calP(E)$ encodes features $f\in E'$ w.r.t. $F$ if $\mu(F)=f$. This notion is particularly useful when $E'=E$ and $F(x)=x$ in which case $\delta_x(F)=x$, and $\delta_x$ encodes feature $x$. This will allow us to translate notions about vector-space representations to notions about measures and the features they encode.

Moreover, we can parameterize families of measures by the features they encode. Let \mbox{$F:E\to E'$} be fixed, and suppose we have identified a mapping $f\mapsto \nu_f\in \calP(E)$ which is a bijection \aristide{ injection, no?} and for which $\nu_f(F)=f$. Then we denote by $\calF_F=\{\nu_f\st f\in E'\}$ the family of all such distributions, usually omitting the subscript $F$ when there is no chance of confusion. Two particular cases are a natural exponential family with sufficient statistics $F$, and $\calP_\delta(E)$ for $E'=E$ and $F(x)=x$. We will consider both in the sequel. Finally, we define the feature projection onto $\calF$, denoted $\Pi_\calF:\calP(E)\to \calF$, defined by
\[
	\Pi_\calF(\mu) = \nu_{\mu(F)}.
\]{\todo This mapping will allow us to represent finite-dimensional features with measures while keeping the dimensionality of such representations finite.}

==> preamble.tex <==


% The following packages will be automatically loaded:
% amsmath, amssymb, natbib, graphicx, url, algorithm2e
\usepackage{amsmath, amssymb, natbib, graphicx, url, algorithm2e, amsthm}
\usepackage{geometry}
\usepackage{tocloft}

% \usepackage{mdframed}

\usepackage{thmtools,thm-restate}
\usepackage{{James}}
\newcommand{\attn}{\mathrm{Attention}}
\newcommand{\ffn}{\mathrm{FFN}}
\newcommand{\layernorm}{\mathrm{LayerNorm}}
\newcommand{\resnorm}{\mathrm{ResNorm}}
\newcommand{\multiattn}{\mathrm{MultiHeadAttention}}
\newcommand{\multiselfattn}{\mathrm{MultiHeadSelfAttention}}
\newcommand{\selfattn}{\mathrm{SelfAttention}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\softmatch}{\mathrm{softmatch}}
% \newcommand{\encoder}{\mathrm{Encoder}}
\newcommand{\transf}{\mathrm{Transformer}}
\newcommand{\attnkern}{\mathrm{AttentionKernel}}

\newcommand{\eps}{\epsilon}
\newcommand{\bdot}{\bullet}

\newcommand{\E}{\mathds{E}}
\newcommand{\N}{\mathds{N}}
\newcommand{\M}{\mathds{M}}
\newcommand{\K}{\mathds{K}}
\renewcommand{\P}{\mathds{P}}
\renewcommand{\Q}{\mathds{Q}}
\newcommand{\T}{\mathds{T}
\newcommand{\V}{\mathds{V}}
\newcommand{\X}{\mathds{X}}
\newcommand{\Y}{\mathds{Y}}
\newcommand{\W}{\mathds{W}}
\newcommand{\KL}{\mathds{KL}}

\newcommand{\diam}{\mathrm{diam}}

\newcommand{\scrF}{\mathscr{F}}

\newcommand{\gremph}[1]{{\color{gray}#1}}
\newcommand{\remph}[1]{{\color{red}#1}}
\newcommand{\qeq}{\overset{?}{=}}
\newcommand{\eqd}{\overset{d}{=}}
\newcommand{\mmbf}[1]{\ensuremath{\boldsymbol #1}}
\newcommand{\defn}[1]{\textbf{#1}}

\newtheorem*{assumption*}{Assumption}
\newtheorem*{claim}{Claim}
\newtheorem{example}{Example}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{axiom}[theorem]{Axiom}
\newcommand{\james}[1]{{\color{blue}\textbf{[James:]}#1}}
\newcommand{\remi}[1]{{\color{red}\textbf{[Remi:]}#1}}
\newcommand{\aristide}[1]{{\color{green}\textbf{[Aristide:]}#1}}

